A Systematic Mapping Study of Code Quality in Education -- with Complete Bibliography

While functionality and correctness of code has traditionally been the main focus of computing educators, quality aspects of code are getting increasingly more attention. High-quality code contributes to the maintainability of software systems, and should therefore be a central aspect of computing education. We have conducted a systematic mapping study to give a broad overview of the research conducted in the field of code quality in an educational context. The study investigates paper characteristics, topics, research methods, and the targeted programming languages. We found 195 publications (1976-2022) on the topic in multiple databases, which we systematically coded to answer the research questions. This paper reports on the results and identifies developments, trends, and new opportunities for research in the field of code quality in computing education.

==> arxiv sources/full-table.tex <==
"I know it when i see it" - Perceptions of code quality,  \citeauthor{927} \cite{927} & 2018 & Perceptions & DescrCorr & generic &  &  &  & rd &  &  \\ 
A card game for learning software-refactoring principles,  \citeauthor{8} \cite{8} & 2019 & Materials & Survey & generic-OO & cs &  &  &  & rf &  \\ 
A case study of the analysis of novice student programs,  \citeauthor{10} \cite{10} & 1999 & ProgramQuality & DescrCorr & C++ &  &  & mt &  &  & sa \\ 
A case study of the static analysis of the quality of novice student programs,  \citeauthor{11} \cite{11} & 1999 & ProgramQuality & DescrCorr & C++ &  &  & mt &  &  & sa \\ 
A critic for LISP,  \citeauthor{fischer1987} \cite{fischer1987} & 1987 & SelfmadeTool & Tool & Lisp &  &  &  &  &  &  \\ 
A design quality learning unit in OO modeling bridging the engineer and the artist,  \citeauthor{34} \cite{34} & 2011 & Curriculum & NoneUnclear & generic-OO &  &  & mt &  &  &  \\ 
A diagnosis system of programming styles using program patterns,  \citeauthor{37} \cite{37} & 2000 & SelfmadeTool & (Q)Experim & C &  &  &  & rd &  &  \\ 
A framework for the assessment and training of software refactoring competences,  \citeauthor{47} \cite{47} & 2019 & Curriculum & CaseStudy & generic &  &  &  &  & rf &  \\ 
A Heuristic Tool for Measuring Software Quality Using Program Language Standards,  \citeauthor{n153} \cite{n153} & 2022 & SelfmadeTool & Tool & Java &  &  &  &  &  &  \\ 
A Large-Scale Comparison of Python Code in Jupyter Notebooks and Scripts,  \citeauthor{n261} \cite{n261} & 2022 & ProgramQuality & DescrCorr & Python &  &  &  &  &  &  \\ 
A method for detecting bad smells and ITS application to software engineering education,  \citeauthor{59} \cite{59} & 2014 & SelfmadeTool & Tool & Java & cs &  &  &  & rf &  \\ 
A pedagogical approach in interleaving software quality concerns at an artificial intelligence course,  \citeauthor{n107} \cite{n107} & 2022 & TeachingMethod & NoneUnclear & Java &  &  & mt &  &  &  \\ 
A programming style taxonomy,  \citeauthor{92} \cite{92} & 1991 & Assignments & Other & generic &  &  &  &  &  &  \\ 
A Proposal of Coding Rule Learning Function in Java Programming Learning Assistant System,  \citeauthor{94} \cite{94} & 2016 & SelfmadeTool & Survey & Java &  &  &  & rd &  & sa \\ 
A Resource to Support Novices Refactoring Conditional Statements,  \citeauthor{n55} \cite{n55} & 2022 & TeachingMethod & (Q)Experim & C & cs &  &  & rd & rf &  \\ 
A study of loop style and abstraction in pedagogic practice,  \citeauthor{125} \cite{125} & 2011 & ProgramQuality & Qualitative & mutiple &  &  &  &  &  &  \\ 
A study on the quality mindedness of students,  \citeauthor{n217} \cite{n217} & 2022 & Perceptions & Survey & generic &  &  &  &  &  &  \\ 
A tool for diagnosing the quality of java program and a method for its effective utilization in education,  \citeauthor{149} \cite{149} & 2010 & ExternalTool & (Q)Experim & Java &  &  &  & rd &  &  \\ 
A Tutoring System to Learn Code Refactoring,  \citeauthor{n297} \cite{n297} & 2021 & SelfmadeTool & Tool & Java &  &  &  &  & rf &  \\ 
Academic coding guideline model - OCG,  \citeauthor{169} \cite{169} & 2014 & Assignments & Discussion & C &  &  &  & rd &  &  \\ 
Amelioration of Teaching Strategies by Exploring Code Quality and Submission Behavior,  \citeauthor{197} \cite{197} & 2019 & Behaviour & DescrCorr & C++ & cs &  &  &  &  &  \\ 
An Agile classroom experience: Teaching TDD and refactoring,  \citeauthor{200} \cite{200} & 2008 & ProgProcess & Experience & Java &  &  &  &  & rf &  \\ 
An Applicability Study on Refactoring Principles in Reading-Based Programming Learning,  \citeauthor{n257} \cite{n257} & 2022 & Materials & (Q)Experim & Java &  & dp &  &  & rf &  \\ 
An automated assessment system for analysis of coding convention violations in Java programming assignments,  \citeauthor{212} \cite{212} & 2018 & SelfmadeTool & Tool & Java &  &  &  & rd &  &  \\ 
An Automatic Grading System for a High School-level Computational Thinking Course,  \citeauthor{n263} \cite{n263} & 2022 & SelfmadeTool & QuantOther & Haskell &  &  &  &  &  &  \\ 
An empirical study of COBOL programs via a style analyzer: The benefits of good programming style,  \citeauthor{224} \cite{224} & 1989 & Behaviour & DescrCorr & Cobol &  &  & mt &  &  &  \\ 
An empirical study of iterative improvement in programming assignments,  \citeauthor{225} \cite{225} & 2015 & Behaviour & DescrCorr & C++ &  &  & mt &  &  &  \\ 
An empirical study on students' ability to comprehend design patterns,  \citeauthor{232} \cite{232} & 2008 & ConceptUnd & (Q)Experim & mutiple &  & dp & mt &  &  &  \\ 
An Incremental Model for Developing Educational Critiquing Systems: Experiences with the Java Critiquer,  \citeauthor{b3} \cite{b3} & 2008 & SelfmadeTool & DescrCorr & Java &  &  &  &  &  &  \\ 
An innovative approach to teaching refactoring,  \citeauthor{266} \cite{266} & 2006 & ProgProcess & NoneUnclear & generic-OO &  &  &  &  & rf &  \\ 
An instructional aid for student programs,  \citeauthor{267} \cite{267} & 1980 & SelfmadeTool & DescrCorr & Fortran &  &  &  &  &  &  \\ 
Analysis of Learning Behavior in an Automated Programming Assessment Environment: A Code Quality Perspective,  \citeauthor{292} \cite{292} & 2020 & Behaviour & QuantOther & Java &  &  &  &  &  &  \\ 
Analyzing students' software redesign strategies,  \citeauthor{300} \cite{300} & 2016 & Behaviour & Qualitative & Java &  & dp &  &  & rf &  \\ 
Anomaly Detection for Early Warning in Object-oriented Programming Course,  \citeauthor{n319} \cite{n319} & 2021 & SelfmadeTool & Tool & Java &  &  &  &  &  & sa \\ 
Applying Code Quality Detection in Online Programming Judge,  \citeauthor{317} \cite{317} & 2020 & ExternalTool & DescrCorr & Python &  &  &  &  &  &  \\ 
Applying gamification to motivate students to write high-quality code in programming assignments,  \citeauthor{318} \cite{318} & 2019 & TeachingMethod & (Q)Experim & C &  &  & mt &  &  &  \\ 
Are Undergraduate Creative Coders Clean Coders? A Correlation Study,  \citeauthor{n302} \cite{n302} & 2022 & ProgramQuality & DescrCorr & Java &  &  &  &  &  &  \\ 
ASPA: A Static Analyser to Support Learning and Continuous Feedback on Programming Courses. An Empirical Validation,  \citeauthor{n275} \cite{n275} & 2022 & SelfmadeTool & Survey & Python &  &  &  &  &  & sa \\ 
Assessing software quality of agile student projects by data-mining software repositories,  \citeauthor{349} \cite{349} & 2019 & ProgramQuality & DescrCorr & unknown &  &  & mt &  &  &  \\ 
Assessing the quality of programs: A topic for the CS2 course,  \citeauthor{sanders1987} \cite{sanders1987} & 1987 & ProgramQuality & Discussion & generic &  &  &  &  &  &  \\ 
Assessing Understanding of Maintainability using Code Review,  \citeauthor{n16} \cite{n16} & 2021 & Assignments & (Q)Experim & generic &  &  &  &  &  &  \\ 
Automated critique of early programming antipatterns,  \citeauthor{366} \cite{366} & 2019 & SelfmadeTool & Tool & Java &  &  &  &  &  & sa \\ 
Automatic analysis of functional program style,  \citeauthor{michaelson1996} \cite{michaelson1996} & 1996 & SelfmadeTool & Tool & SML &  &  &  &  &  &  \\ 
Automatic assessment aids for Pascal programs,  \citeauthor{rees1982} \cite{rees1982} & 1982 & SelfmadeTool & DescrCorr & Pascal &  &  &  &  &  &  \\ 
Automatic Assessment of the Design Quality of Student Python and Java Programs,  \citeauthor{n178} \cite{n178} & 2022 & SelfmadeTool & (Q)Experim & mutiple &  &  &  & rd &  &  \\ 
Automatic detection of bad programming habits in scratch,  \citeauthor{moreno2014} \cite{moreno2014} & 2014 & ProgramQuality & DescrCorr & Scratch &  &  &  &  &  &  \\ 
Automatic grader for programming assignment using source code analyzer,  \citeauthor{375} \cite{375} & 2014 & SelfmadeTool & DescrCorr & mutiple &  &  &  &  &  &  \\ 
Automatic programming assessment,  \citeauthor{377} \cite{377} & 1993 & ProgramQuality & DescrCorr & Pascal &  &  & mt &  &  &  \\ 
AutoStyle: Toward coding style feedback at scale,  \citeauthor{386} \cite{386} & 2015 & SelfmadeTool & Tool & mutiple &  &  &  &  &  &  \\ 
Bad Smells in Scratch Projects: A Preliminary Analysis,  \citeauthor{vargas2019} \cite{vargas2019} & 2019 & ProgramQuality & DescrCorr & Scratch & cs &  &  &  &  &  \\ 
Beautiful JavaScript: How to guide students to create good and elegant code,  \citeauthor{387} \cite{387} & 2014 & ProgProcess & NoneUnclear & JavaScript &  &  &  &  & rf &  \\ 
Beauty and the Beast: on the readability of object-oriented example programs,  \citeauthor{388} \cite{388} & 2016 & Materials & DescrCorr & Java &  &  &  & rd &  &  \\ 
But my program runs! Discourse rules for novice programmers,  \citeauthor{Joni86} \cite{Joni86} & 1986 & Assignments & NoneUnclear & Pascal &  &  &  &  &  &  \\ 
Can students help themselves? An investigation of students' feedback on the quality of the source code,  \citeauthor{410} \cite{410} & 2019 & ProgramQuality & Survey & Python &  &  &  &  &  &  \\ 
Carrot and Stick approaches revisited when managing Technical Debt in an educational context,  \citeauthor{Crespo21} \cite{Crespo21} & 2021 & TeachingMethod & (Q)Experim & Java &  &  & mt &  &  &  \\ 
Challenges of knowledge component modeling: A software engineering case study,  \citeauthor{n161} \cite{n161} & 2022 & Materials & CaseStudy & generic &  &  &  &  & rf &  \\ 
Clean Code - Delivering A Lightweight Course,  \citeauthor{n243} \cite{n243} & 2021 & TeachingMethod & NoneUnclear & Java &  &  &  &  &  &  \\ 
Clean Code and Design Educational Tool,  \citeauthor{n1} \cite{n1} & 2021 & SelfmadeTool & Tool & C\# & cs &  &  & rd &  &  \\ 
Clean Code Tutoring: Makings of a Foundation,  \citeauthor{n155} \cite{n155} & 2022 & SelfmadeTool & (Q)Experim & C\# &  &  &  & rd & rf &  \\ 
Cleangame: Gamifying the identification of code smells,  \citeauthor{442} \cite{442} & 2019 & SelfmadeTool & (Q)Experim & Java & cs &  &  &  & rf &  \\ 
Code Comprehension Activities in Undergraduate Software Engineering Course - A Case Study,  \citeauthor{449} \cite{449} & 2015 & Behaviour & DescrCorr & mutiple &  &  &  &  & rf &  \\ 
Code Perfumes: Reporting Good Code to Encourage Learners,  \citeauthor{n18} \cite{n18} & 2021 & ProgramQuality & DescrCorr & Scratch & cs &  &  &  &  &  \\ 
Code Quality Defects Across Introductory Programming Topics,  \citeauthor{n303} \cite{n303} & 2022 & ProgramQuality & DescrCorr & Python &  &  &  &  &  &  \\ 
Code Quality Improvement for All: Automated Refactoring for Scratch,  \citeauthor{452} \cite{452} & 2019 & SelfmadeTool & (Q)Experim & Scratch & cs &  & mt &  & rf &  \\ 
Code quality issues in student programs,  \citeauthor{453} \cite{453} & 2017 & ProgramQuality & DescrCorr & Java &  &  &  &  &  &  \\ 
Code quality: Examining the efficacy of automated tools,  \citeauthor{454} \cite{454} & 2017 & ExternalTool & DescrCorr & Python &  &  & mt &  &  &  \\ 
CompareCFG: Providing Visual Feedback on Code Quality Using Control Flow Graphs,  \citeauthor{487} \cite{487} & 2020 & SelfmadeTool & Tool & Java &  &  &  &  &  &  \\ 
Comparison of software quality in the work of children and professional developers based on their classroom exercises,  \citeauthor{493} \cite{493} & 2015 & ProgramQuality & DescrCorr & Java &  &  &  &  &  &  \\ 
Comprehension and application of design patterns by novice software engineers,  \citeauthor{499} \cite{499} & 2018 & ConceptUnd & (Q)Experim & Java &  & dp &  &  &  &  \\ 
Dependency Analysis for Learning Class Structure for Novice Java Programmer,  \citeauthor{558} \cite{558} & 2011 & TeachingMethod & CaseStudy & Java &  &  &  & rd & rf &  \\ 
Design of e-activities for the learning of code refactoring tasks,  \citeauthor{571} \cite{571} & 2014 & TeachingMethod & Experience & generic &  &  &  &  & rf &  \\ 
Design patterns in scientific software,  \citeauthor{575} \cite{575} & 2004 & TeachingMethod & NoneUnclear & Java &  & dp &  &  & rf &  \\ 
Designing a Programming Game to Improve Children's Procedural Abstraction Skills in Scratch,  \citeauthor{580} \cite{580} & 2020 & SelfmadeTool & (Q)Experim & Scratch & cs &  &  &  &  &  \\ 
Designing a rubric for feedback on code quality in programming courses,  \citeauthor{581} \cite{581} & 2016 & Assignments & Other & generic &  &  &  &  &  &  \\ 
Detecting and Addressing Design Smells in Novice Processing Programs,  \citeauthor{591} \cite{591} & 2019 & ProgramQuality & DescrCorr & Processing & cs &  &  &  & rf & sa \\ 
Development of a refactoring learning environment,  \citeauthor{605} \cite{605} & 2011 & SelfmadeTool & Tool & Java &  &  &  &  & rf &  \\ 
Do code smells hamper novice programming? A controlled experiment on Scratch programs,  \citeauthor{623} \cite{623} & 2016 & ConceptUnd & (Q)Experim & Scratch & cs &  &  &  &  &  \\ 
Documentation Standards for Beginning Students,  \citeauthor{628} \cite{628} & 1976 & Assignments & NoneUnclear & mutiple &  &  &  & rd &  &  \\ 
Does Static Analysis Help Software Engineering Students?,  \citeauthor{634} \cite{634} & 2020 & ExternalTool & DescrCorr & Java &  &  &  &  &  & sa \\ 
Dr. Scratch: Automatic analysis of scratch projects to assess and foster computational thinking,  \citeauthor{moreno2015dr} \cite{moreno2015dr} & 2015 & SelfmadeTool & (Q)Experim & Scratch &  &  &  &  &  &  \\ 
DrPython-WEB: A Tool to Help Teaching Well-Written Python Programs,  \citeauthor{n209} \cite{n209} & 2022 & SelfmadeTool & Tool & Python &  &  &  &  &  &  \\ 
Earthworm - Automated decomposition suggestions,  \citeauthor{647} \cite{647} & 2018 & SelfmadeTool & Tool & Python &  &  &  &  & rf & sa \\ 
Effectively teaching coding standards in programming,  \citeauthor{li2005} \cite{li2005} & 2005 & Perceptions & Survey & generic &  &  &  &  &  &  \\ 
Effects of technical debt awareness: A classroom study,  \citeauthor{tonin2017} \cite{tonin2017} & 2017 & TeachingMethod & Qualitative & generic &  &  &  &  &  &  \\ 
Encapsulation and Reuse as Viewed by Java Students,  \citeauthor{b17} \cite{b17} & 2001 & Perceptions & Qualitative & Java &  &  &  &  &  &  \\ 
Enhancing Abstraction in App Inventor with Generic Event Handlers,  \citeauthor{patton2019} \cite{patton2019} & 2019 & SelfmadeTool & Tool & APPInventor & cs &  &  &  & rf &  \\ 
Enhancing block-based programming pedagogy to promote the culture of quality from the ground up - a position paper,  \citeauthor{712} \cite{712} & 2017 & Curriculum & Discussion & generic-block &  &  &  &  &  &  \\ 
Evaluating Code Improvements in Software Quality Course Projects,  \citeauthor{n24} \cite{n24} & 2022 & TeachingMethod & (Q)Experim & Java &  &  &  &  &  & sa \\ 
Evolving an integrated curriculum for object-oriented analysis and design,  \citeauthor{ramnath2008} \cite{ramnath2008} & 2008 & Curriculum & Experience & generic-OO &  & dp &  &  & rf &  \\ 
Exploration of Experimental Teaching Reforms on C Programming Design Course,  \citeauthor{n255} \cite{n255} & 2021 & TeachingMethod & DescrCorr & C &  &  &  &  &  &  \\ 
Exploring Metrics for the Analysis of Code Submissions in an Introductory Data Science Course,  \citeauthor{Nguyen21} \cite{Nguyen21} & 2021 & ProgramQuality & DescrCorr & Python &  &  & mt &  &  &  \\ 
Five reasons for including technical debt in the software engineering curriculum,  \citeauthor{falessi2015} \cite{falessi2015} & 2015 & Curriculum & NoneUnclear & generic &  &  &  &  &  &  \\ 
Foobaz: Variable name feedback for student code at scale,  \citeauthor{824} \cite{824} & 2015 & SelfmadeTool & Survey & Python &  &  &  &  &  &  \\ 
Forming groups for collaborative learning in introductory computer programming courses based on students' programming styles: An empirical study,  \citeauthor{829} \cite{829} & 2006 & ProgProcess & (Q)Experim & C &  &  & mt &  &  &  \\ 
Fostering the comprehension of the object-oriented programming paradigm by a virtual lab exercise,  \citeauthor{thurner2019} \cite{thurner2019} & 2019 & TeachingMethod & Experience & Java &  &  &  &  &  &  \\ 
FrenchPress gives students automated feedback on Java program flaws,  \citeauthor{835} \cite{835} & 2015 & SelfmadeTool & Survey & Java &  &  &  &  &  &  \\ 
Function Names: Quantifying the Relationship Between Identifiers and Their Functionality to Improve Them,  \citeauthor{n337} \cite{n337} & 2022 & SelfmadeTool & Tool & Java &  &  &  & rd &  &  \\ 
Gamification based learning environment for computer science students,  \citeauthor{853} \cite{853} & 2020 & SelfmadeTool & Tool & mutiple &  &  &  &  &  & sa \\ 
Helping Student Programmers Through Industrial-Strength Static Analysis: A Replication Study,  \citeauthor{n304} \cite{n304} & 2022 & Behaviour & DescrCorr & Java &  &  &  &  &  & sa \\ 
High School Teachers' Understanding of Code Style,  \citeauthor{893} \cite{893} & 2020 & Perceptions & Qualitative & generic &  &  &  &  &  &  \\ 
How junior developers deal with their technical debt?,  \citeauthor{910} \cite{910} & 2020 & Behaviour & Mixed & mutiple &  &  &  &  &  & sa \\ 
How kids code and how we know: An exploratory study on the scratch repository,  \citeauthor{911} \cite{911} & 2016 & ProgramQuality & DescrCorr & Scratch & cs &  &  &  &  &  \\ 
How teachers would help students to improve their code,  \citeauthor{917} \cite{917} & 2019 & ProgramQuality & Survey & generic &  &  &  &  &  &  \\ 
How to improve code quality by measurement and refactoring,  \citeauthor{918} \cite{918} & 2016 & ProgProcess & DescrCorr & Java &  &  & mt &  & rf & sa \\ 
Human vs. Automated coding style grading in computing education,  \citeauthor{924} \cite{924} & 2019 & ProgramQuality & DescrCorr & C++ &  &  &  &  &  & sa \\ 
Hyperstyle: A Tool for Assessing the Code Quality of Solutions to Programming Assignments,  \citeauthor{n305} \cite{n305} & 2022 & SelfmadeTool & Tool & mutiple &  &  &  & rd & rf &  \\ 
Impact of aspect-oriented programming on the quality of novices' programs: A comparative study,  \citeauthor{939} \cite{939} & 2013 & ProgramQuality & (Q)Experim & C\# &  &  & mt & rd &  &  \\ 
Implementing a set of guidelines for CS majors in the production of program code,  \citeauthor{poole1996} \cite{poole1996} & 1996 & Assignments & Survey & Modula2 &  &  &  &  &  &  \\ 
Improving Feedback on GitHub Pull Requests: A Bots Approach,  \citeauthor{957} \cite{957} & 2019 & SelfmadeTool & Mixed & generic-OO & cs &  &  &  &  & sa \\ 
Improving Readability of Scratch Programs with Search-based Refactoring,  \citeauthor{n272} \cite{n272} & 2021 & SelfmadeTool & Tool & Scratch &  &  &  & rd & rf &  \\ 
Improving students programming quality with the continuous inspection process: a social coding perspective,  \citeauthor{968} \cite{968} & 2019 & ProgProcess & (Q)Experim & Java &  &  &  &  &  &  \\ 
Improving the software quality - An educational approach,  \citeauthor{974} \cite{974} & 2017 & SelfmadeTool & Tool & C\# &  & dp &  &  & rf &  \\ 
Integrating Antipatterns into the Computer Science Curriculum,  \citeauthor{1005} \cite{1005} & 2009 & Curriculum & NoneUnclear & generic-OO &  & dp &  &  & rf &  \\ 
Investigating code quality tools in the context of software engineering education,  \citeauthor{1028} \cite{1028} & 2017 & ExternalTool & DescrCorr & Java &  &  & mt &  & rf &  \\ 
Investigating static analysis errors in student Java programs,  \citeauthor{1032} \cite{1032} & 2017 & ProgramQuality & DescrCorr & Java &  &  &  &  &  & sa \\ 
Investigation of the relationship between program correctness and programming style,  \citeauthor{1041} \cite{1041} & 1999 & ProgramQuality & DescrCorr & mutiple &  &  & mt & rd &  &  \\ 
Japroch: A tool for checking programming style,  \citeauthor{makela2004} \cite{makela2004} & 2004 & SelfmadeTool & Tool & Java &  &  &  &  &  &  \\ 
JMetricGrader: A software for evaluating student projects using design object-oriented metrics and neural networks,  \citeauthor{n8} \cite{n8} & 2022 & ProgramQuality & QuantOther & Java &  &  & mt &  &  &  \\ 
Learning appreciation for design patterns by doing it the hard way first,  \citeauthor{skrien2003} \cite{skrien2003} & 2003 & TeachingMethod & Experience & Java &  & dp &  &  & rf &  \\ 
Learning software engineering principles using open source software,  \citeauthor{1079} \cite{1079} & 2008 & Assignments & NoneUnclear & Java &  &  & mt & rd & rf &  \\ 
Learning to listen for design,  \citeauthor{1083} \cite{1083} & 2019 & ProgProcess & Discussion & generic & cs & dp &  &  & rf &  \\ 
Linking code readability, structure, and comprehension among novices: It's complicated,  \citeauthor{1091} \cite{1091} & 2019 & Perceptions & Survey & mutiple &  &  &  & rd &  &  \\ 
Litterbox: A linter for scratch programs,  \citeauthor{Fraser21} \cite{Fraser21} & 2021 & SelfmadeTool & Tool & Scratch & cs &  &  &  &  &  \\ 
Measuring static quality of student code,  \citeauthor{1121} \cite{1121} & 2011 & ProgramQuality & DescrCorr & Java &  &  & mt &  &  &  \\ 
Measuring students' source code quality in software development projects through commit-impact analysis,  \citeauthor{Hamer21} \cite{Hamer21} & 2021 & Behaviour & DescrCorr & mutiple &  &  & mt &  &  &  \\ 
Mind the Gap: Searching for Clarity in NCEA,  \citeauthor{n58} \cite{n58} & 2021 & Materials & Mixed & generic &  &  &  &  &  &  \\ 
Mining student CVS repositories for performance indicators,  \citeauthor{1145} \cite{1145} & 2005 & Behaviour & DescrCorr & mutiple &  &  &  &  &  &  \\ 
Modeling Learners Programming Skills and Question Levels Through Machine Learning,  \citeauthor{1160} \cite{1160} & 2020 & ProgramQuality & QuantOther & mutiple &  &  &  & rd &  &  \\ 
Novice Programmers and Software Quality: Trends and Implications,  \citeauthor{1190} \cite{1190} & 2017 & ProgramQuality & DescrCorr & Scratch & cs &  &  &  &  &  \\ 
On assuring learning about code quality,  \citeauthor{1201} \cite{1201} & 2020 & Curriculum & CaseStudy & generic &  &  &  &  &  &  \\ 
On the Use of FCA Models in Static Analysis Tools to Detect Common Errors in Programming,  \citeauthor{n213} \cite{n213} & 2021 & ProgramQuality & DescrCorr & Python &  &  &  &  &  & sa \\ 
Pirate plunder: Game-based computational thinking using scratch blocks,  \citeauthor{1268} \cite{1268} & 2018 & SelfmadeTool & Tool & Scratch & cs &  &  &  &  &  \\ 
Program decomposition and complexity in CS1,  \citeauthor{1310} \cite{1310} & 2015 & TeachingMethod & (Q)Experim & C &  &  & mt &  &  &  \\ 
Programming style in introductory programming courses,  \citeauthor{1320} \cite{1320} & 2015 & Curriculum & NoneUnclear & generic &  &  &  &  &  &  \\ 
Promoting Code Quality via Automated Feedback on Student Submissions,  \citeauthor{n267} \cite{n267} & 2021 & SelfmadeTool & Tool & mutiple &  &  &  &  &  &  \\ 
Qualitative aspects of students' programs: Can we make them measurable?,  \citeauthor{1337} \cite{1337} & 2016 & SelfmadeTool & (Q)Experim & Python &  &  &  &  &  &  \\ 
Quality Assessment of Learners' Programs by Grouping Source Code Metrics,  \citeauthor{n156} \cite{n156} & 2021 & ProgramQuality & QuantOther & Lua &  &  & mt &  &  &  \\ 
Readable vs. Writable Code: A Survey of Intermediate Students' Structure Choices,  \citeauthor{n347} \cite{n347} & 2022 & Perceptions & Survey & Java &  &  &  & rd &  &  \\ 
RefacTutor: An Interactive Tutoring System for Software Refactoring,  \citeauthor{1432} \cite{1432} & 2020 & SelfmadeTool & Tool & Java &  &  &  &  & rf &  \\ 
Reflections on teaching refactoring: A tale of two projects,  \citeauthor{1433} \cite{1433} & 2015 & ProgProcess & (Q)Experim & Java &  &  &  &  &  &  \\ 
ReLE - a refactoring supporting tool,  \citeauthor{1437} \cite{1437} & 2011 & SelfmadeTool & Tool & Java &  &  &  &  & rf &  \\ 
Replicating novices' struggles with coding style,  \citeauthor{1442} \cite{1442} & 2019 & Perceptions & Survey & mutiple &  &  &  & rd &  &  \\ 
Research and practice on education of SQA at source code level,  \citeauthor{1449} \cite{1449} & 2011 & TeachingMethod & CaseStudy & generic &  &  &  &  &  &  \\ 
Salient elements in novice solutions to code writing problems,  \citeauthor{1478} \cite{1478} & 2011 & ProgramQuality & Qualitative & mutiple &  &  &  &  &  &  \\ 
Scale-driven automatic hint generation for coding style,  \citeauthor{1479} \cite{1479} & 2016 & SelfmadeTool & (Q)Experim & mutiple &  &  &  &  &  &  \\ 
Serious refactoring games,  \citeauthor{haendler2019} \cite{haendler2019} & 2019 & Materials & NoneUnclear & generic-OO & cs &  &  &  & rf &  \\ 
Smells in block-based programming languages,  \citeauthor{1517} \cite{1517} & 2016 & ProgramQuality & DescrCorr & generic-block & cs &  &  &  &  &  \\ 
Software analytics to support students in object-oriented programming tasks: an empirical study,  \citeauthor{ardimento2020} \cite{ardimento2020} & 2020 & ProgramQuality & (Q)Experim & Java &  &  &  &  &  &  \\ 
Software clones in scratch projects: On the presence of copy-and-paste in computational thinking learning,  \citeauthor{robles2017} \cite{robles2017} & 2017 & ProgramQuality & DescrCorr & Scratch &  &  &  &  &  &  \\ 
Software engineer education support system ALECSS utilizing devOps tools,  \citeauthor{1532} \cite{1532} & 2016 & SelfmadeTool & DescrCorr & Java &  &  &  &  &  & sa \\ 
Software metrics as a programming training tool,  \citeauthor{1545} \cite{1545} & 1990 & Assignments & (Q)Experim & Cobol &  &  & mt &  &  &  \\ 
Software Quality as a Subsidy for Teaching Programming,  \citeauthor{n268} \cite{n268} & 2021 & TeachingMethod & DescrCorr & Java &  &  &  &  &  &  \\ 
Software Quality Metrics Calculations for Java Programming Learning Assistant System,  \citeauthor{1574} \cite{1574} & 2020 & SelfmadeTool & DescrCorr & Java &  &  & mt &  &  &  \\ 
Software readability practices and the importance of their teaching,  \citeauthor{1581} \cite{1581} & 2016 & Assignments & Survey & generic-OO & cs &  &  & rd &  &  \\ 
Sprinter: A Didactic Linter for Structured Programming,  \citeauthor{Alfredo22} \cite{Alfredo22} & 2022 & SelfmadeTool & Tool & Java &  &  &  &  &  &  \\ 
Static analyses in python programming courses,  \citeauthor{1617} \cite{1617} & 2019 & SelfmadeTool & (Q)Experim & Python &  &  &  &  &  & sa \\ 
Static analysis of programming exercises: Fairness, usefulness and a method for application,  \citeauthor{1620} \cite{1620} & 2016 & ExternalTool & DescrCorr & Java &  &  &  &  &  & sa \\ 
Static analysis of source code written by novice programmers,  \citeauthor{1621} \cite{1621} & 2017 & ExternalTool & DescrCorr & C &  &  &  &  &  & sa \\ 
Static Analysis of Students' Java Programs,  \citeauthor{1622} \cite{1622} & 2004 & SelfmadeTool & Tool & Java &  &  & mt &  &  & sa \\ 
Structural analysis of source code collected from programming contests,  \citeauthor{1632} \cite{1632} & 2014 & ProgramQuality & QuantOther & C++ &  &  &  &  &  &  \\ 
Student Refactoring Behaviour in a Programming Tutor,  \citeauthor{1643} \cite{1643} & 2020 & Behaviour & DescrCorr & Java &  &  &  &  & rf &  \\ 
Students Projects' Source Code Changes Impact on Software Quality Through Static Analysis,  \citeauthor{n93} \cite{n93} & 2021 & Behaviour & DescrCorr & mutiple &  &  &  &  &  & sa \\ 
Studying Software Metrics Based on Real-World Software Systems,  \citeauthor{1658} \cite{1658} & 2007 & Assignments & NoneUnclear & generic &  &  & mt &  &  &  \\ 
Supporting Students in C++ Programming Courses with Automatic Program Style Assessment,  \citeauthor{b42} \cite{b42} & 2004 & SelfmadeTool & Qualitative & C++ &  &  &  &  &  &  \\ 
Teacher Mate: A Support Tool for Teaching Code Quality,  \citeauthor{1675} \cite{1675} & 2020 & SelfmadeTool & DescrCorr & Java &  &  &  &  &  &  \\ 
Teaching code quality in high school programming courses - Understanding teachers' needs,  \citeauthor{n30} \cite{n30} & 2022 & Perceptions & Qualitative & generic &  &  &  &  &  &  \\ 
Teaching Defensive Programming in Java,  \citeauthor{1692} \cite{1692} & 2004 & Assignments & Survey & Java &  &  &  &  &  &  \\ 
Teaching design patterns using a family of games,  \citeauthor{1693} \cite{1693} & 2009 & Assignments & Experience & Java &  & dp &  &  & rf &  \\ 
Teaching programming style with ugly code,  \citeauthor{1704} \cite{1704} & 2013 & SelfmadeTool & Tool & Java &  &  &  & rd &  &  \\ 
Teaching software quality via source code inspection tool,  \citeauthor{1720} \cite{1720} & 2017 & SelfmadeTool & (Q)Experim & mutiple &  &  &  &  &  &  \\ 
Teaching students to build well formed object-oriented methods through refactoring,  \citeauthor{1729} \cite{1729} & 2007 & ProgProcess & NoneUnclear & generic-OO &  &  &  &  & rf &  \\ 
Teaching students to recognize and implement good coding style,  \citeauthor{1730} \cite{1730} & 2017 & ProgramQuality & (Q)Experim & Python &  &  &  &  &  &  \\ 
Teaching the culture of quality from the ground up: Novice-tailored quality improvement for scratch programmers,  \citeauthor{tilevich2020} \cite{tilevich2020} & 2020 & SelfmadeTool & Mixed & Scratch &  &  &  &  & rf &  \\ 
The effect of reporting Known issues on students' work,  \citeauthor{1782} \cite{1782} & 2018 & Perceptions & (Q)Experim & C++ &  &  &  &  &  &  \\ 
The Five Million Piece Puzzle: Finding Answers in 500,000 Snap-Projects,  \citeauthor{1790} \cite{1790} & 2019 & ProgramQuality & DescrCorr & Snap! & cs &  &  &  &  &  \\ 
The impact of automated code quality feedback in programming education,  \citeauthor{1796} \cite{1796} & 2017 & ExternalTool & (Q)Experim & mutiple &  &  &  &  &  &  \\ 
The LAN-simulation: A refactoring teaching example,  \citeauthor{1807} \cite{1807} & 2005 & Assignments & Experience & Java &  &  &  &  & rf &  \\ 
The Role of Source Code Vocabulary in Programming Teaching and Learning,  \citeauthor{1824} \cite{1824} & 2020 & SelfmadeTool & (Q)Experim & Python &  &  &  & rd &  &  \\ 
The teaching of documentation and good programming style in a liberal arts computer science program,  \citeauthor{1830} \cite{1830} & 1980 & TeachingMethod & NoneUnclear & Basic &  &  &  &  &  &  \\ 
Tool assisted identifier naming for improved software readability: An empirical study,  \citeauthor{1854} \cite{1854} & 2005 & SelfmadeTool & (Q)Experim & Java &  &  &  & rd &  &  \\ 
Towards an empirically validated model for assessment of code quality,  \citeauthor{1875} \cite{1875} & 2014 & Assignments & Qualitative & generic &  &  &  &  &  &  \\ 
Towards generalizing expert programmers' suggestions for novice programmers,  \citeauthor{1880} \cite{1880} & 2013 & ProgramQuality & Survey & Alice-LG &  &  &  &  &  & sa \\ 
Understanding recurring quality problems and their impact on code sharing in block-based software,  \citeauthor{1908} \cite{1908} & 2017 & ProgramQuality & DescrCorr & Scratch & cs &  &  &  &  &  \\ 
Understanding Refactoring Tasks over Time: A Study Using Refactoring Graphs,  \citeauthor{n88} \cite{n88} & 2022 & Behaviour & (Q)Experim & Java &  &  &  &  & rf &  \\ 
Understanding Semantic Style by Analysing Student Code,  \citeauthor{1909} \cite{1909} & 2018 & ProgramQuality & DescrCorr & Java &  &  &  &  &  &  \\ 
Unencapsulated collection - A teachable design smell,  \citeauthor{1912} \cite{1912} & 2018 & ProgramQuality & CaseStudy & generic-OO & cs &  &  &  & rf &  \\ 
Unreadable code in novice developers,  \citeauthor{Avila21} \cite{Avila21} & 2021 & Perceptions & Survey & generic &  &  &  & rd &  &  \\ 
Using examples as guideposts for programming exercises: Providing support while preserving the challenge,  \citeauthor{n126} \cite{n126} & 2021 & Assignments & CaseStudy & C++ &  &  &  &  & rf &  \\ 
Using pirate plunder to develop children's abstraction skills in scratch,  \citeauthor{1951} \cite{1951} & 2019 & SelfmadeTool & (Q)Experim & Scratch & cs &  &  &  &  &  \\ 
Using project-based approach to teach design patterns: An Experience Report,  \citeauthor{n33} \cite{n33} & 2021 & TeachingMethod & (Q)Experim & Java & cs & dp &  &  & rf &  \\ 
Using software metrics tools for maintenance decisions: a classroom exercise,  \citeauthor{1954} \cite{1954} & 1996 & ExternalTool & CaseStudy & unknown &  &  & mt &  &  &  \\ 
Using static analysis tools to assist student project evaluation,  \citeauthor{1956} \cite{1956} & 2020 & ExternalTool & DescrCorr & Python &  &  &  &  &  & sa \\ 
Using Verilog LOGISCOPE to analyze student programs,  \citeauthor{1964} \cite{1964} & 1998 & ExternalTool & DescrCorr & C++ &  &  &  &  &  & sa \\ 
Utilizing software engineering education support system ALECSS at an actual software development experiment: A case study,  \citeauthor{1967} \cite{1967} & 2019 & SelfmadeTool & DescrCorr & Java &  &  &  &  &  &  \\ 
You have said too much : Java-like verbosity anti-patterns in python codebases,  \citeauthor{n311} \cite{n311} & 2021 & ProgramQuality & DescrCorr & Python &  &  &  &  &  &  \\ 

